PromptSmooth: Certifying Robustness of Medical Vision-Language Models via Prompt Learning

Medical vision-language models (Med-VLMs) trained on large datasets of medical image-text pairs and later fine-tuned for specific tasks have emerged as a mainstream paradigm in medical image analysis. However, recent studies have highlighted the susceptibility of these Med-VLMs to adversarial attacks, raising concerns about their safety and robustness. Randomized smoothing is a well-known technique for turning any classifier into a model that is certifiably robust to adversarial perturbations. However, this approach requires retraining the Med-VLM-based classifier so that it classifies well under Gaussian noise, which is often infeasible in practice. In this paper, we propose a novel framework called PromptSmooth to achieve efficient certified robustness of Med-VLMs by leveraging the concept of prompt learning. Given any pre-trained Med-VLM, PromptSmooth adapts it to handle Gaussian noise by learning textual prompts in a zero-shot or few-shot manner, achieving a delicate balance between accuracy and robustness, while minimizing the computational overhead. Moreover, PromptSmooth requires only a single model to handle multiple noise levels, which substantially reduces the computational cost compared to traditional methods that rely on training a separate model for each noise level. Comprehensive experiments based on three Med-VLMs and across six downstream datasets of various imaging modalities demonstrate the efficacy of PromptSmooth. Our code and models are available at https://github.com/nhussein/promptsmooth.

==> tables/certify_plip_kather.tex <==
\begin{table}[t]
\centering
\caption{\small Comparison of best certified accuracy per radius of zero-shot PLIP, our \texttt{PromptSmooth} methods, CoOp, baselines: Denoised Smoothing and Diffusion Denoiser, on 500 samples from all 9 classes of KatherColon test set at various $\ell_2$ radii. (The number within parentheses at the top left corner indicates the certified accuracy at $R=0$, representing the standard accuracy.)}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\rowcolor{gray!20} \textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1.0 & 1.25 & 1.5 \\
\midrule
Zero-shot PLIP & $^{(56.6)}$49.4 & $^{(56.6)}$38.2 & $^{(28.9)}$20.8 & $^{(28.9)}$17.6 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 \\
% Denoised Smoothing$^\text{(mse\_obj)}$ & $^{(48.6)}$38.6 & $^{(48.6)}$28.8 & $^{(27.6)}$25.0 & $^{(27.6)}$22.6 & $^{(27.6)}$18.6 & $^{(22.4)}$13.0 & $^{(22.4)}$12.0 \\
% Denoised Smoothing$^\text{(clf+stab+obj)}$ & $^{(52.4)}$47.2 & $^{(52.4)}$39.8 & $^{(44.2)}$29.4 & $^{(44.2)}$22.6 & $^{(28.0)}$17.0 & $^{(28.0)}$15.8 & $^{(28.0)}$14.2 \\
%$^\text{(stab+mse\_obj)}$
Denoised Smoothing \cite{salman2020denoised} & $^{(55.0)}$48.2 & $^{(55.0)}$39.2 & $^{(45.2)}$31.0 & $^{(45.2)}$25.6 & $^{(26.2)}$17.4 & $^{(26.2)}$16.2 & $^{(26.2)}$14.6 \\
Diffusion Smoothing \cite{carlini2022certified} & $^{(58.0)}$57.0 & $^{(53.0)}$49.0 & $^{(53.0)}$41.0	& $^{(53.0)}$34.0 & $^{(53.0)}$26.0 & $^{(53.0)}$22.0	& $^{(53.0)}$16.0 \\
\rowcolor{Apricot!20} \texttt{Zero-shot PromptSmooth} & $^{(57.6)}$53.4 & $^{(57.6)}$49.0 & $^{(30.2)}$29.0 & $^{(30.2)}$29.0 & $^{(30.2)}$28.6 & $^{(30.2)}$28.4 & $^{(30.2)}$27.4 \\
\midrule
CoOp \cite{zhou2022learning} & $^{(71.6)}$66.7 & $^{(71.6)}$56 & $^{(22.0)}$16.4 & $^{(22.0)}$14.2 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 \\
Denoised Smoothing + CoOp & $^{(38.0)}$36.2 & $^{(38.0)}$ 30.6 & $^{(34.0)}$24.4	& $^{(34.0)}$17.8 & $^{(11.0)}$11.0	& $^{(11.0)}$11.0	& $^{(11.0)}$11.0	\\
Diffusion Smoothing + CoOp & $^{(79.0)}$74.0 & $^{(70.0)}$64.0 & $^{(66.0)}$57.0 & $^{(66.0)}$54.0 & $^{(60.0)}$\textbf{49.0} & $^{(60.0)}$45.0 & $^{(60.0)}$44.0 \\
% \rowcolor{orange!6} Few-shot PromptSmooth (separate noise)& $^{(74.6)}$72.2 & $^{(74.6)}$66.6 & $^{(62.8)}$48.2 & $^{(62.8)}$36.6 & $^{(26.0)}$19.4 & $^{(26.0)}$14.4 & $^{(26.0)}$11.6 \\
\rowcolor{Apricot!20}  \texttt{Few-Shot PromptSmooth} & $^{(81.2)}$78.2 & $^{(81.2)}$67.6 & $^{(75.6)}$52.2 & $^{(75.6)}$35.6 & $^{(50.4)}$26.4 & $^{(50.4)}$22.2 & $^{(50.4)}$17.6 \\
% \rowcolor{orange!6} PromptSmooth (separate noise) & $^{(75.4)}$74.6 & $^{(75.4)}$74.0 & $^{(68.4)}$67.2 & $^{(68.4)}$65.0 & $^{(19.2)}$19.0 & $^{(19.2)}$19.0 & $^{(19.2)}$19.0 \\
\midrule
\rowcolor{Apricot!20} \texttt{PromptSmooth}& $^{(82.0)}$\textbf{81.8} & $^{(82.0)}$\textbf{81.0} & $^{(76.6)}$\textbf{74.8} & $^{(76.6)}$\textbf{73.2} & $^{(54.0)}$48.4 & $^{(54.0)}$\textbf{47.2} & $^{(54.0)}$\textbf{45.6} \\
\bottomrule
\end{tabular}
}
\label{tab:plip_kather_results}
\end{table}

==> tables/ctx_init_tpt.tex <==
\begin{wraptable}{r}{0.5\linewidth}
\vspace{-0.7cm}
\caption{\small Zero-shot PromptSmooth context initialization}
\resizebox{\linewidth}{!}{\begin{tabular}{@{}l*{5}{c}@{}}
\toprule
\rowcolor{gray!20}\textbf{Caption} & \multicolumn{5}{r}{\textbf{Certification at $\ell_2$ Radius}} \\
\cmidrule(l){2-6} & 0 & 0.1 & 0.25 & 0.5 & 0.75 \\
\midrule
'An H\&E image patch of' & 38.0 & 35.0 & 32.0& 31.0 & 23.0 \\
'An H\&E noisy image patch of' & 40.0 & 38.0 & 38.0 & 35.0 & 34.0 \\
\bottomrule
\end{tabular}}
\label{tab:promptsmooth-init}
\end{wraptable}


==> tables/merged.tex <==
\begin{table}[t]
\centering
\caption{Comparison of best certified accuracy per radius of \textbf{zero-shot PLIP} (ViT-B/32), \textbf{Baselines}, \textbf{Zero-shot PromptSmooth}, \textbf{Few-shot PrmptSmooth}  and \textbf{PromptSmooth} on 500 samples from 9 different classes of KatherColon test set at various $\ell_2$ radii. $N_0 = 100$ and $N = 10,000$. (The number within parentheses at the top left corner indicates the certified accuracy at $R=0$, representing the standard accuracy.)}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\textbf{Method} \multicolumn{3}{l}& \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1.0 & 1.25 & 1.5 \\
\midrule
 Zero-shot PLIP \multicolumn{3}{l} & $^{(56.6)}$49.4 & $^{(56.6)}$38.2 & $^{(28.9)}$20.8 & $^{(28.9)}$17.6 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 \\
%Denoised Smoothing $^\text{(mse\_obj)}$ \multicolumn{3}{l}  & $^{(48.6)}$38.6 & $^{(48.6)}$28.8 & $^{(27.6)}$25.0 & $^{(27.6)}$22.6 & $^{(27.6)}$18.6 & $^{(22.4)}$13.0 & $^{(22.4)}$12.0 \\
%Denoised Smoothing $^\text{(clf+stab+obj)}$ \multicolumn{3}{l} & $^{(52.4)}$47.2 & $^{(52.4)}$39.8 & $^{(44.2)}$29.4 & $^{(44.2)}$22.6 & $^{(28.0)}$17.0 & $^{(28.0)}$15.8 & $^{(28.0)}$14.2 \\
%$^\text{(stab+mse\_obj)}$
Denoised Smoothing \multicolumn{3}{l}  & $^{(55.0)}$48.2 & $^{(55.0)}$39.2 & $^{(45.2)}$31.0 & $^{(45.2)}$25.6 & $^{(26.2)}$17.4 & $^{(26.2)}$16.2 & $^{(26.2)}$14.6 \\
Diffusion Denoiser \multicolumn{3}{l}& $^{(58.0)}$57.0 & $^{(53.0)}$49.0 & $^{(53.0)}$41.0	& $^{(53.0)}$34.0 & $^{(53.0)}$26.0 & $^{(53.0)}$22.0	& $^{(53.0)}$16.0 \\
\midrule
\texttt{Zero-shot PromptSmooth} \multicolumn{3}{l} & $^{(57.6)}$53.4 & $^{(57.6)}$49.0 & $^{(30.2)}$29.0 & $^{(30.2)}$29.0 & $^{(30.2)}$28.6 & $^{(30.2)}$28.4 & $^{(30.2)}$27.4 \\
\midrule
\midrule
CoOp \multicolumn{3}{l} & $^{(71.6)}$66.7 & $^{(71.6)}$56 & $^{(22.0)}$16.4 & $^{(22.0)}$14.2 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 & $^{(11.0)}$11.0 \\
Denoised Smoothing + CoOp \multicolumn{3}{l} & $^{(38.0)}$36.2 & $^{(38.0)}$ 30.6 & $^{(34.0)}$24.4	& $^{(34.0)}$17.8 & $^{(11.0)}$11.0	& $^{(11.0)}$11.0	& $^{(11.0)}$11.0	\\
 Diffusion Denoiser + CoOp \multicolumn{3}{l}& $^{(79.0)}$74.0 & $^{(70.0)}$64.0 & $^{(66.0)}$57.0 & $^{(66.0)}$54.0 & $^{(60.0)}$\textbf{49.0} & $^{(60.0)}$45.0 & $^{(60.0)}$44.0 \\
\midrule
% \rowcolor{orange!6} Few-shot PromptSmooth (separate noise)& $^{(74.6)}$72.2 & $^{(74.6)}$66.6 & $^{(62.8)}$48.2 & $^{(62.8)}$36.6 & $^{(26.0)}$19.4 & $^{(26.0)}$14.4 & $^{(26.0)}$11.6 \\
\rowcolor{Apricot!20} \texttt{Few-Shot PromptSmooth} \multicolumn{3}{l} & $^{(81.2)}$78.2 & $^{(81.2)}$67.6 & $^{(75.6)}$52.2 & $^{(75.6)}$35.6 & $^{(50.4)}$26.4 & $^{(50.4)}$22.2 & $^{(50.4)}$17.6 \\
% \rowcolor{orange!6} PromptSmooth (separate noise) & $^{(75.4)}$74.6 & $^{(75.4)}$74.0 & $^{(68.4)}$67.2 & $^{(68.4)}$65.0 & $^{(19.2)}$19.0 & $^{(19.2)}$19.0 & $^{(19.2)}$19.0 \\
\rowcolor{Apricot!20} \texttt{PromptSmooth} \multicolumn{3}{l}& $^{(82.0)}$\textbf{81.8} & $^{(82.0)}$\textbf{81.0} & $^{(76.6)}$\textbf{74.8} & $^{(76.6)}$\textbf{73.2} & $^{(54.0)}$48.4 & $^{(54.0)}$\textbf{47.2} & $^{(54.0)}$\textbf{45.6} \\
% \bottomrule
% \end{tabular}
% \label{tab:plip_kather_results}
% \end{table}
% \begin{tabular}{@{}lccccccccc@{}}
\midrule
\textbf{Method} & \multicolumn{4}{c}{\textbf{COVID19}} & & \multicolumn{4}{c}{\textbf{RSNA18}} \\
\cmidrule(lr){2-5} \cmidrule(lr){7-10}
& 0.1 & 0.25 & 0.5 & 0.75 & & 0.1 & 0.25 & 0.5 & 0.75 \\
\midrule
Denoised Smoothing & $^{(66.4)}$54.6 & $^{(50.2)}$48.4 & $^{(50.2)}$45.8 & $^{(50.2)}$36.0 & & $^{(37.6)}$27.6 & $^{(31.6)}$21.0 & $^{(31.6)}$9.40 & $^{(31.6)}$1.79 \\
Diffusion Denoiser & $^{(56.0)}$37.0 & $^{(44.0)}$22.0 & $^{(44.0)}$6.00 & $^{(44.0)}$1.00 & & $^{(44.0)}$40.0 & $^{(44.0)}$28.0 & $^{(44.0)}$12.0 & $^{(44.0)}$1.00 \\
\texttt{Zero-shot PromptSmooth} & $^{(62.4)}$62.0 & $^{(62.4)}$60.6 & $^{(50.2)}$50.0 & $^{(50.2)}$49.8 & & $^{(37.0)}$35.4 & $^{(37.0)}$33.4 & $^{(33.4)}$33.4 & $^{(33.4)}$\textbf{33.2} \\
\texttt{Few-shot PromptSmooth} & $^{(66.8)}$58.0 & $^{(52.0)}$48.8 & $^{(52.0)}$47.6 & $^{(52)}$42.8 & & $^{(41.4)}$34.4 & $^{(34.0)}$31.2 & $^{(34.0)}$27.0 & $^{(34.0)}$23.6 \\
\midrule
\rowcolor{Apricot!20} \texttt{PromptSmooth} & $^{(69.4)}$\textbf{69.0} & $^{(69.4)}$\textbf{68.4} & $^{(53.0)}$\textbf{52.8} & $^{(53.0)}$\textbf{52.6} & & $^{(42.4)}$\textbf{40.8} & $^{(42.4)}$\textbf{35.8} & $^{(34.6)}$\textbf{33.4} & $^{(34.6)}$32.0 \\
\bottomrule

\end{tabular}}
\label{tab:merged_tables}
\end{table}


==> tables/original_tpt_aug.tex <==
\begin{wraptable}{r}{0.55\linewidth}
\centering
\caption{\small Comparison of Original TPT augmentations versus Zero-shot PromptSmooth method at various $\ell_2$ radii.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
% \rowcolor{gray!20}\textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ Radius (\%)}} \\
%  \cmidrule(l){2-8} & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
% \midrule
% TPT Augmentations & $^{(46.8)}$43.2 & $^{(46.8)}$37.6 & $^{(25.4)}$21.2 & $^{(25.4)}$17.8 & $^{(15.4)}$11.0 & $^{(15.4)}$10.6 & $^{(15.4)}$10.2 \\
% Zero-shot PromptSmooth & $^{(57.6)}$\textbf{53.4} & $^{(57.6)}$\textbf{49.0} & $^{(30.2)}$\textbf{29.0} & $^{(30.2)}$\textbf{29.0} & $^{(30.2)}$\textbf{28.6} & $^{(30.2)}$\textbf{28.4} & $^{(30.2)}$\textbf{27.4} \\
\rowcolor{gray!20}\textbf{Method} & \multicolumn{3}{c}{\textbf{Certified Accuracy at $\ell_2$ Radius (\%)}} \\
\cmidrule(l){2-4} & 0.5 & 1.0 & 1.5 \\
\midrule
TPT Augmentations & $^{(25.4)}$21.2 & $^{(15.4)}$11.0 & $^{(15.4)}$10.2 \\
Zero-shot PromptSmooth & $^{(30.2)}$\textbf{29.0} &  $^{(30.2)}$\textbf{28.6} &  $^{(30.2)}$\textbf{27.4} \\
\bottomrule
\end{tabular}
}
\label{tab:tpt-vs-promptsmooth}
\end{wraptable}



==> tables/plip_3_datasets.tex <==
\begin{table}[h]
\centering
\caption{\small Certification results of PLIP on 3 datasets for undefended zero-shot PLIP, naive prompt-tuning and our proposed \texttt{PromptSmooth} methods.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\rowcolor{gray!20} \textbf{Dataset / Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ radius (\%)}} \\
\rowcolor{gray!20} & 0.1 & 0.25 & 0.5 & 0.75 & 1.0 & 1.25 & 1.5 \\
\midrule
\multicolumn{8}{c}{\textbf{PanNuke (Binary)}} \\
\midrule
Zero-shot PLIP & $^{(59.6)}$55.8 & $^{(52)}$50.8 & $^{(52)}$50.2 & $^{(50.2)}$50.0 & $^{(50.2)}$50.0 & $^{(50.2)}$50.0 & $^{(50.2)}$50.0 \\
Naive Approach (CoOp) \cite{zhou2022learning} & $^{(73.6)}$69.8 & $^{(73.6)}$61.8 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 \\
\rowcolor{Apricot!20} Zero-shot PromptSmooth & $^{(51.6)}$51.4 & $^{(51.6)}$51.4 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 \\
\rowcolor{Apricot!20} Few-shot PromptSmooth & $^{(73.2)}$68.8 & $^{(73.2)}$58.8 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 \\
\rowcolor{Apricot!20} PromptSmooth & $^{(73.8)}$\textbf{73.8 }& $^{(73.8)}$\textbf{73.8 }& $^{(68.8)}$\textbf{68.8} & $^{(68.8)}$\textbf{68.8} & $^{(65.2)}$\textbf{65.2} & $^{(65.2)}$\textbf{65.2} & $^{(65.2)}$\textbf{65.2} \\
\midrule
\multicolumn{8}{c}{\textbf{SICAPv2 (4 Classes)}} \\
\midrule
Zero-shot PLIP & $^{(43.2)}$40.0 & $^{(43.2)}$33.6 & $^{(25.0)}$25.5 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
Naive Approach (CoOp) \cite{zhou2022learning} & $^{(45.0)}$37.0 & $^{(45.0)}$27.2 & $^{(25.0)}$25.5 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
\rowcolor{Apricot!20} Zero-shot PromptSmooth & $^{(44.2)}$42.8 & $^{(44.2)}$39.6 & $^{(44.2)}$33.8 & $^{(44.2)}$27.8 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
\rowcolor{Apricot!20} Few-shot PromptSmooth & $^{(51.4)}$40.0 & $^{(51.4)}$26.6 & $^{(27.8)}$15.8 & $^{(27.8)}$10.8 & $^{(27.8)}$7.40 & $^{(27.8)}$4.40 & $^{(27.8)}$2.00 \\
\rowcolor{Apricot!20} PromptSmooth & $^{(51.6)}$\textbf{50.8} & $^{(51.6)}$\textbf{49.6} & $^{(46.8)}$\textbf{39.4} & $^{(46.8)}$\textbf{35.0} & $^{(46.8)}$\textbf{30.2} & $^{(46.8)}$\textbf{30.0} & $^{(46.8)}$\textbf{28.2} \\
\midrule
\multicolumn{8}{c}{\textbf{SkinCancer (16 Classes)}} \\
\midrule
Zero-shot PLIP & $^{(26.6)}$19.0 & $^{(14.2)}$9.80 & $^{(6.0)}$5.80 & $^{(6.00)}$4.80 & $^{(6.00)}$4.60 & $^{(6.00)}$4.39 & $^{(6.00)}$4.39 \\
Naive Approach (CoOp) \cite{zhou2022learning} & $^{(67.2)}$57.8 & $^{(67.2)}$43.8 & $^{(34.2)}$16.6 & $^{(34.2)}$7.00 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 \\
\rowcolor{Apricot!20} Zero-shot PromptSmooth & $^{(25)}$23.2 & $^{(25)}$19.6 & $^{(14.2)}$11.6 & $^{(6.40)}$6.40 & $^{(6.40)}$6.40 & $^{(6.40)}$6.40 & $^{(6.40)}$6.40 \\
\rowcolor{Apricot!20} Few-shot PromptSmooth & $^{(67.0)}$58.0 & $^{(67.0)}$44.6 & $^{(54.4)}$27.0 & $^{(36.6)}$15.0 & $^{(36.6)}$9.00 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 \\
\rowcolor{Apricot!20} PromptSmooth & $^{(68.6)}$\textbf{67.6} & $^{(68.6)}$\textbf{64.8} & $^{(56.4)}$\textbf{50.2} & $^{(56.4)}$\textbf{46.0} & $^{(38.2)}$\textbf{33.8} & $^{(38.2)}$\textbf{31.0}& $^{(38.2)}$\textbf{29.6} \\
\bottomrule
\end{tabular}
}
\label{tab:combined-results}
\end{table}

==> tables/plip_pannuke.tex <==
\begin{table}[t]
\centering
\caption{\small Results on PanNuke (binary) dataset for various $\ell_2$ radii. The numbers in parentheses represent the standard accuracy.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ Radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
\midrule
Zero-shot PLIP & $^{(59.6)}$55.8 & $^{(52)}$50.8 & $^{(52)}$50.2 & $^{(50.2)}$50.0 & $^{(50.2)}$50.0 & $^{(50.2)}$50.0 & $^{(50.2)}$50.0 \\
Zero-shot PromptSmooth & $^{(51.6)}$51.4 & $^{(51.6)}$51.4 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 & $^{(50.6)}$50.6 \\
CoOp & $^{(73.6)}$69.8 & $^{(73.6)}$61.8 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 \\
Few-shot PromptSmooth & $^{(73.2)}$68.8 & $^{(73.2)}$58.8 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 & $^{(50.0)}$50.0 \\
PromptSmooth & $^{(73.8)}$\textbf{73.8 }& $^{(73.8)}$\textbf{73.8 }& $^{(68.8)}$\textbf{68.8} & $^{(68.8)}$\textbf{68.8} & $^{(65.2)}$\textbf{65.2} & $^{(65.2)}$\textbf{65.2} & $^{(65.2)}$\textbf{65.2} \\
\bottomrule
\end{tabular}
}
\label{tab:pannuke-results}
\end{table}

==> tables/plip_sicapv2.tex <==
\begin{table}[t]
\centering
\caption{\small Results on SICAPv2 (4 classes) dataset for various $\ell_2$ radii. The numbers in parentheses represent the standard accuracy.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ Radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
\midrule
Zero-shot PLIP & $^{(43.2)}$40.0 & $^{(43.2)}$33.6 & $^{(25.0)}$25.5 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
Zero-shot PromptSmooth & $^{(44.2)}$42.8 & $^{(44.2)}$39.6 & $^{(44.2)}$33.8 & $^{(44.2)}$27.8 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
CoOp & $^{(45.0)}$37.0 & $^{(45.0)}$27.2 & $^{(25.0)}$25.5 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
Few-shot PromptSmooth & $^{(51.4)}$40.0 & $^{(51.4)}$26.6 & $^{(27.8)}$15.8 & $^{(27.8)}$10.8 & $^{(27.8)}$7.39 & $^{(27.8)}$4.39 & $^{(27.8)}$2.00 \\
PromptSmooth & $^{(51.6)}$\textbf{50.8} & $^{(51.6)}$\textbf{49.6} & $^{(46.8)}$\textbf{39.4} & $^{(46.8)}$\textbf{35.0} & $^{(46.8)}$\textbf{30.2} & $^{(46.8)}$\textbf{30.0} & $^{(46.8)}$\textbf{28.2} \\
\bottomrule
\end{tabular}
}
\label{tab:sicapv2-results}
\end{table}

==> tables/plip_skincancer.tex <==
\begin{table}[t]
\centering
\caption{\small Results on SkinCancer (16 classes) dataset for various $\ell_2$ radii. The numbers in parentheses represent the standard accuracy.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ Radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
\midrule
Zero-shot PLIP & $^{(26.6)}$19.0 & $^{(14.2)}$9.80 & $^{(6.0)}$5.80 & $^{(6.00)}$4.80 & $^{(6.00)}$4.60 & $^{(6.00)}$4.39 & $^{(6.00)}$4.39 \\
Zero-shot PromptSmooth & $^{(25)}$23.2 & $^{(25)}$19.6 & $^{(14.2)}$11.6 & $^{(6.40)}$6.40 & $^{(6.40)}$6.40 & $^{(6.40)}$6.40 & $^{(6.40)}$6.40 \\
CoOp & $^{(67.2)}$57.8 & $^{(67.2)}$43.8 & $^{(34.2)}$16.6 & $^{(34.2)}$7.00 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 \\
Few-shot PromptSmooth & $^{(67.0)}$58.0 & $^{(67.0)}$44.6 & $^{(54.4)}$27.0 & $^{(36.6)}$15.0 & $^{(36.6)}$9.00 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 \\
PromptSmooth & $^{(68.6)}$\textbf{67.6} & $^{(68.6)}$\textbf{64.8} & $^{(56.4)}$\textbf{50.2} & $^{(56.4)}$\textbf{46.0} & $^{(38.2)}$\textbf{33.8} & $^{(38.2)}$\textbf{31.0}& $^{(38.2)}$\textbf{29.6} \\
\bottomrule
\end{tabular}
}
\label{tab:skincancer-results}
\end{table}


==> tables/quilt_2_datasets.tex <==
\begin{table}[h]
\centering
\caption{\small Certification results of Quilt on 2 datasets for undefended zero-shot Quilt, naive prompt-tuning and our proposed \texttt{PromptSmooth} methods.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\rowcolor{gray!20} \textbf{Datasets / Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ radius (\%)}} \\
\rowcolor{gray!20} & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
\midrule
\multicolumn{8}{c}{\textbf{SICAPv2 (4 Classes)}}\\
\midrule
Zero-shot Quilt & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25)}$25.0 & $^{(25)}$24.6 & $^{(25)}$24.2 & $^{(25)}$23.8 \\
Naive Approach (CoOp) \cite{zhou2022learning} & $^{(55.8)}$47.2 & $^{(55.8)}$35.8 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
\rowcolor{Apricot!20} Zero-shot Promptsmooth & $^{(25.8)}$25.8 & $^{(25.8)}$25.6 & $^{(25.8)}$25.6 & $^{(25.8)}$25.2 & $^{(25.8)}$25.0 & $^{(25.8)}$24.8 & $^{(25.8)}$24.8 \\
\rowcolor{Apricot!20} Few-shot PromptSmooth & $^{(62.0)}$49.8 & $^{(62.0)}$31.8 & $^{(31.2)}$17.0 & $^{(31.2)}$10.8 & $^{(31.2)}$6.40 & $^{(31.2)}$2.60 & $^{(31.2)}$0.60 \\
\rowcolor{Apricot!20} PromptSmooth & $^{(60.0)}$\textbf{59.0} & $^{(60.0)}$\textbf{57.0} & $^{(55.4)}$\textbf{49.8} & $^{(55.4)}$\textbf{46.8} & $^{(32.2)}$\textbf{31.0} & $^{(32.2)}$\textbf{30.6} & $^{(32.2)}$\textbf{30.6} \\
\midrule
\multicolumn{8}{c}{\textbf{SkinCancer (16 Classes)}} \\
\midrule
Zero-shot Quilt & $^{(33.0)}$25.8 & $^{(33.0)}$15.8 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 \\
Naive Approach (CoOp) \cite{zhou2022learning} & $^{(52.8)}$43.2 & $^{(52.8)}$31.0 & $^{(18.2)}$7.60 & $^{(6.80)}$6.20 & $^{(6.80)}$6.20 & $^{(6.80)}$6.20 & $^{(6.80)}$6.20 \\
\rowcolor{Apricot!20} Zero-shot PromptSmooth & $^{(29.2)}$26.4 & $^{(29.2)}$20.6 & $^{(14.79)}$9.80 & $^{(14.79)}$6.60 & $^{(4.20)}$3.20 & $^{(4.20)}$3.20 & $^{(4.20)}$2.40 \\
\rowcolor{Apricot!20} Few-shot PromptSmooth & $^{(69.4)}$61.0 & $^{(64.4)}$51.0 & $^{(64.4)}$53.0 & $^{(64.4)}$35.0 & $^{(64.4)}$17.6 & $^{(46.0)}$9.20 & $^{(46.0)}$3.80 \\
\rowcolor{Apricot!20} PromptSmooth & $^{(71.0)}$\textbf{70.0} & $^{(71.0)}$\textbf{67.0} & $^{(66.2)}$\textbf{62.0} & $^{(66.2)}$\textbf{57.8} & $^{(46.8)}$\textbf{42.6} & $^{(46.8)}$\textbf{41.6} & $^{(46.8)}$\textbf{40.6} \\
\bottomrule
\end{tabular}
}
\label{tab:quilt_datasets}
\end{table}

==> tables/quilt_sicapv2.tex <==
\begin{table}[t]
\centering
\caption{\small Results on SICAPv2 (4 classes) dataset for various $\ell_2$ radii. The numbers in parentheses represent the standard accuracy.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
\midrule
Zero-shot Quilt & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25)}$25.0 & $^{(25)}$24.6 & $^{(25)}$24.2 & $^{(25)}$23.8 \\
Zero-shot Promptsmooth & $^{(25.8)}$25.8 & $^{(25.8)}$25.6 & $^{(25.8)}$25.6 & $^{(25.8)}$25.2 & $^{(25.8)}$25.0 & $^{(25.8)}$24.8 & $^{(25.8)}$24.8 \\
Clean CoOp & $^{(55.8)}$47.2 & $^{(55.8)}$35.8 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 & $^{(25.0)}$25.0 \\
Few-shot PromptSmooth & $^{(62.0)}$49.8 & $^{(62.0)}$31.8 & $^{(31.2)}$17.0 & $^{(31.2)}$10.8 & $^{(31.2)}$6.40 & $^{(31.2)}$2.60 & $^{(31.2)}$0.60 \\
PromptSmooth & $^{(60.0)}$\textbf{59.0} & $^{(60.0)}$\textbf{57.0} & $^{(55.4)}$\textbf{49.8} & $^{(55.4)}$\textbf{46.8} & $^{(32.2)}$\textbf{31.0} & $^{(32.2)}$\textbf{30.6} & $^{(32.2)}$\textbf{30.6} \\
\bottomrule
\end{tabular}
}
\label{tab:sicapv2-results}
\end{table}


==> tables/quilt_skincancer.tex <==
\begin{table}[t]
\centering
\caption{\small Results on SkinCancer (16 classes) dataset for various $\ell_2$ radii. The numbers in parentheses represent the standard accuracy.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \multicolumn{7}{c}{\textbf{Certified Accuracy at $\ell_2$ radius (\%)}} \\
\cmidrule(l){2-8}
 & 0.1 & 0.25 & 0.5 & 0.75 & 1 & 1.25 & 1.5 \\
\midrule
Zero-shot Quilt & $^{(33.0)}$25.8 & $^{(33.0)}$15.8 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 & $^{(6.20)}$6.20 \\
CoOp & $^{(52.8)}$43.2 & $^{(52.8)}$31.0 & $^{(18.2)}$7.60 & $^{(6.80)}$6.20 & $^{(6.80)}$6.20 & $^{(6.80)}$6.20 & $^{(6.80)}$6.20 \\
Zero-shot PromptSmooth & $^{(29.2)}$26.4 & $^{(29.2)}$20.6 & $^{(14.79)}$9.80 & $^{(14.79)}$6.60 & $^{(4.20)}$3.20 & $^{(4.20)}$3.20 & $^{(4.20)}$2.40 \\
Few-shot PromptSmooth & $^{(69.39)}$61.0 & $^{(64.4)}$51.0 & $^{(64.4)}$53.0 & $^{(64.4)}$35.0 & $^{(64.4)}$17.6 & $^{(46.0)}$9.20 & $^{(46.0)}$3.80 \\
PromptSmooth & $^{(71.0)}$\textbf{70.0} & $^{(71.0)}$\textbf{67.0} & $^{(66.2)}$\textbf{62.0} & $^{(66.2)}$\textbf{57.8} & $^{(46.8)}$\textbf{42.6} & $^{(46.8)}$\textbf{41.6} & $^{(46.8)}$\textbf{40.6} \\
\bottomrule
\end{tabular}
}
\label{tab:skincancer-results}
\end{table}

